Braiding on type A Soergel bimodules: semistrictness and naturality

We consider categories of Soergel bimodules for the symmetric groups S_n in their gl(n)-realizations for all n and assemble them into a locally linear monoidal bicategory. Chain complexes of Soergel bimodules likewise form a locally dg-monoidal bicategory which can be equipped with the structure of a braiding, whose data includes the Rouquier complexes of shuffle braids. The braiding, together with a uniqueness result, was established in an infinity-categorical setting in recent work with Yu Leon Liu, Aaron Mazel-Gee and David Reutter. In the present article, we construct this braiding explicitly and describe its requisite coherent naturality structure in a concrete dg-model for the morphism categories. To this end, we first assemble the Elias-Khovanov-Williamson diagrammatic Hecke categories as well as categories of chain complexes thereover into locally linear semistrict monoidal 2-categories. Along the way, we prove strictness results for certain standard categorical constructions, which may be of independent interest. In a second step, we provide explicit (higher) homotopies for the naturality of the braiding with respect to generating morphisms of the Elias-Khovanov-Williamson diagrammatic calculus. Rather surprisingly, we observe hereby that higher homotopies appear already for height move relations of generating morphisms. Finally, we extend the homotopy-coherent naturality data for the braiding to all chain complexes using cohomology-vanishing arguments.

==> preamble.tex <==
%auto-ignore
%this ensures the arxiv doesn't try to start TeXing here.
%!TEX root=Naturality.tex

\usepackage{latexsym,exscale,enumitem}
\usepackage{mathtools,amsmath,mathscinet,amsfonts,amssymb,amsthm,bbm,euscript}
\usepackage{amscd, stmaryrd}
\usepackage{ulem}
\usepackage[all]{xy}
%\usepackage[notref,notcite]{showkeys}
\SelectTips{cm}{}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{xcolor}\usepackage{slashbox}
\def\theequation{\arabic{section}.\arabic{equation}}
\usepackage{mathtools}

%%%%%%%%%%% page formatting %%%%%%%%%%%

\addtolength{\hoffset}{-1.6cm}
\addtolength{\textwidth}{3cm}
\hfuzz=6pc


%%%%%%%%%%% hyperref %%%%%%%%%%%

\RequirePackage{color}
\definecolor{references}{rgb}{.7,.1,.6}

\RequirePackage[pdftex,
colorlinks = true,
urlcolor = references, % \href{...}{...} external (URL)
citecolor = references, % \cite{...}
linkcolor = references, % \ref{...} and \pageref{...}
]
{hyperref}
\usepackage{cleveref}

%%%%%%%%%%% tikz %%%%%%%%%%%




%%%%%%%%%%% macros %%%%%%%%%%%

%%% cheat to align different cases or align environments%%%
\newlength{\rightside}
\newcommand*{\rightterm}{}
\newcommand*{\term}[1]{$\textstyle#1$}
\newcommand*{\termd}[1]{$\displaystyle#1$}

%%% color macros %%%

\colorlet{green}{black!30!green}
\newcommand{\BLUE}[1]{\textcolor[rgb]{0.00,0.00,0.80}{#1}}
\newcommand{\GREEN}[1]{\textcolor[rgb]{0.00,0.70,0.00}{#1}}
\newcommand{\RED}[1]{\textcolor[rgb]{0.70,0.00,0.00}{#1}}
\newcommand{\GRAY}[1]{\textcolor[rgb]{0.50,0.50,0.50}{#1}}
\definecolor{CQG}{RGB}{0,153,76}
\definecolor{FS}{RGB}{0,76,153} % foam slice
\def\CQGsgn#1{{\color{CQG}#1}}

%%% bibliography macros %%%

\usepackage[backend=biber,style=alphabetic,maxbibnames=9,doi=false,isbn=false,url=false,maxalphanames=6, giveninits]{biblatex}
\setcounter{biburlnumpenalty}{9000}
\setcounter{biburllcpenalty}{9000}
\setcounter{biburlucpenalty}{8000}
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}
\renewbibmacro*{volume+number+eid}{%
  \printtext{vol.}
  \printfield{volume}%
  \setunit*{\addnbspace}% NEW (optional); there's also \addnbthinspace
  \printfield{number}%
  \setunit{\addcomma\space}%
  \printfield{eid}}
\DeclareFieldFormat[article]{number}{\mkbibparens{#1}}
\usepackage{silence}
% Filter warnings issued by package biblatex starting with "Patching footnotes failed"
\WarningFilter{biblatex}{Patching footnotes failed}
\addbibresource{biblio.bib}


\newcommand{\arxiv}[1]{\href{https://arxiv.org/abs/#1}{\small  arXiv:#1}}
\newcommand{\doi}[1]{\href{https://dx.doi.org/#1}{{\small DOI:#1}}}
\newcommand{\euclid}[1]{\href{https://projecteuclid.org/getRecord?id=#1}{{\small  #1}}}
\newcommand{\mathscinet}[1]{\href{https://www.ams.org/mathscinet-getitem?mr=#1}{\small  #1}}
\newcommand{\googlebooks}[1]{(preview at \href{https://books.google.com/books?id=#1}{google books})}
\newcommand{\notfree}{}
\newcommand{\numdam}[1]{}



%%% abbreviations in italics %%%

\def\emph#1{{\sl #1\/}}
\def\ie{{\sl i.e.\;}}
\def\eg{{\sl e.g.\;}}
\def\Eg{{\sl E.g.\/}}
\def\etc{{\sl etc.\/}}
\def\cf{{\sl c.f.\;}}
\def\etal{\sl{et al.\/}}%
\def\vs{\sl{vs.\/}}%


%%% lazyness macros %%%
\def\cal#1{\mathcal{#1}}
\newcommand{\cat}[1]{\ensuremath{\mbox{\bfseries {\upshape {#1}}}}}
\def\mf#1{\mathfrak{#1}}

\def\lra{{\longrightarrow}}
\let\hat=\widehat
\let\tilde=\widetilde

% arrows

\newcommand{\ra}{\rightarrow} % \PW{duplicate of \to, but keeping because no conflict}

%\newcommand{\la}{\leftarrow} % \PW{not used, conflicts with \la = \lambda}

\newcommand{\xra}{\xrightarrow}

\newcommand{\xla}{\xleftarrow}

\newcommand{\xlra}{\xleftrightarrow}

%\newcommand{\xhookra}[1]{\overset{#1}{\hookra}}

\newcommand{\xhookra}{\xhookrightarrow}
\newcommand{\xhookla}{\xhookleftarrow}

\newcommand{\longla}{\longleftarrow}

\newcommand{\longra}{\longrightarrow}

\newcommand{\xlongra}[1]{\stackrel{#1}{\longra}}
\newcommand{\xlongla}[1]{\stackrel{#1}{\longla}}

\newcommand{\longhookra}{\lhook\joinrel\longrightarrow}
\newcommand{\longhookla}{\longleftarrow\joinrel\rhook}

\newcommand{\xlonghookra}[1]{\stackrel{#1}{\longhookra}}
\newcommand{\xlonghookla}[1]{\stackrel{#1}{\longhookla}}

\newcommand{\squigra}{\rightsquigarrow}

%\newcommand{\op}{\operatorname}
\newcommand{\jj}{\operatorname{j}}
\newcommand{\iso}{\cong}
\newcommand{\maps}{\colon}
\newcommand*{\defeq}{\stackrel{\text{def}}{=}}
\newcommand*{\qis}{\stackrel{\tiny\textrm{q.i.}}{\simeq}}
\newcommand*{\hte}{\stackrel{\text{h.e.}}{\simeq}}
\newcommand*{\htc}{\sim}
\renewcommand{\to}{\rightarrow}
\newcommand{\To}{\Rightarrow}
\newcommand{\TO}{\Rrightarrow}
\newcommand{\scs}{\scriptstyle}
\newcommand{\mm}{\mathrm{m}}

%%% alphabet macros %%%

\def\A{\mathbb{A}}
\def\B{\mathbb{B}}
\def\C{\mathbb{C}}
\def\D{\mathbb{D}}
\renewcommand{\k}{\mathbbm{k}}
\renewcommand{\L}{\mathbb{L}}
\def\N{\mathbb{N}}
\def\Q{\mathbb{Q}}
\def\R{\mathbb{R}}
\def\T{\mathbb{T}}
\def\U{\mathbb{U}}
\def\V{\mathbb{V}}
\def\W{\mathbb{W}}
\def\X{\mathbb{X}}
\def\Y{\mathbb{Y}}
\def\Z{\mathbb{Z}}



\newcommand{\cc}{\mathbf{c}}
\newcommand{\rr}{\mathbf{r}}
\newcommand{\kk}{\mathbf{k}}
\newcommand{\ii}{\mathbf{i}}
\newcommand{\KB}{\mathbf{K}}
\newcommand{\LB}{\mathbf{L}}
\newcommand{\UB}{\mathbf{U}}

\def\cH{\mathcal H}
\def\EE{\mathbb E}

\newcommand{\YC}{\mathcal{Y}}

\newcommand{\AS}{\EuScript A}
\newcommand{\BS}{\EuScript B}
\newcommand{\CS}{\EuScript C}
\newcommand{\DS}{\EuScript D}
\newcommand{\IS}{\EuScript I}
\newcommand{\KS}{\EuScript K}
\newcommand{\MS}{\EuScript M}
\newcommand{\RS}{\EuScript R}
\newcommand{\TS}{\EuScript T}
\newcommand{\US}{\EuScript U}
\newcommand{\USd}{\dot{\EuScript U}}
\newcommand{\VS}{\EuScript V}
\newcommand{\VSred}{\overline{\EuScript V}}
%\newcommand{\VSred}{\EuScript V'}
\newcommand{\WS}{\EuScript W}
\newcommand{\YS}{\EuScript Y}


%%% greek letters %%%


\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\bh}{\hat{\beta}}
\renewcommand{\d}{\delta}
\newcommand{\e}{\varepsilon}
\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\renewcommand{\phi}{\varphi}
\renewcommand{\theta}{\vartheta}

\newcommand{\thickchi}{\mathcal{X}}
\newcommand{\Chi}{\mathfrak{X}}

%%% algebraic structure macros %%%

\newcommand{\sln}{\mf{sl}_n}
\newcommand{\slN}{\mf{sl}_N}
\newcommand{\slm}{\mf{sl}_m}
\newcommand{\slnn}[1]{\mf{sl}_{#1}}

\newcommand{\gln}{\mf{gl}_n}
\newcommand{\glN}{\mf{gl}_N}
\newcommand{\glm}{\mf{gl}_m}
\newcommand{\glnn}[1]{\mf{gl}_{#1}}

\newcommand{\Sbim}{\mathrm{Sbim}} 
\newcommand{\SBim}{\Sbim}
\newcommand{\Sbimcl}{\Sbim}

\newcommand{\BSbim}{\mathrm{BSbim}}
\newcommand{\BSbimcl}{\BSbim}
\newcommand{\BSBim}{\BSbim}


\newcommand{\Hilb}{\mathrm{Hilb}}
\newcommand{\symg}{\mathfrak{S}}


%%% elements, objects, morphisms %%%
%\newcommand{\op}{\operatorname} %%%% Achtung: \operatorname ist wirklich nur für Operatoren geeignet. Stattdessen sollte folgendes funktionieren:
\newcommand{\op}{\mathrm}
\newcommand{\flip}{\operatorname{flip}}
\newcommand{\coev}{\mathrm{coev}}
\newcommand{\del}{\partial}
\newcommand{\E}{{\sf{E}}}
\newcommand{\ev}{\mathrm{ev}}
\newcommand{\F}{{\sf{F}}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\idem}{\mathbbm{1}}
\newcommand{\oone}{\mathbbm{1}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\oonetwo}{_{2}{}\mathbf{1}}
\newcommand{\tr}{\mathrm{tr}}


%%% operator & functor macros %%%

\newcommand{\ad}{\operatorname{ad}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\Braidg}{\operatorname{Br}}
\newcommand{\Ch}{\operatorname{Ch}}
\newcommand{\coker}{{\operatorname{coker}}}
\newcommand{\cone}{\operatorname{cone}}
\newcommand{\convl}{\operatorname{conv}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\END}{\operatorname{END}}
\newcommand{\uEnd}{\underline{\End}}
\newcommand{\Ext}{\operatorname{Ext}}
\newcommand{\FT}{\operatorname{FT}}
\newcommand{\HH}{\operatorname{HH}}
\newcommand{\HHH}{\operatorname{HHH}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\HOM}{\operatorname{HOM}}
\newcommand{\Homcat}{\operatorname{\mathbf{Hom}}}
\newcommand{\Endcat}{\operatorname{\mathbf{End}}}
\newcommand{\uHom}{\underline{\Hom}}
\newcommand{\ido}{{\operatorname{id}}}
\newcommand{\im}{{\operatorname{im}}}
\newcommand{\Ind}{\operatorname{Ind}}
\newcommand{\KhR}{\operatorname{KhR}}
\newcommand{\Kar}{\operatorname{Kar}}
\newcommand{\largewedge}{\mbox{\Large $\wedge$}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\rk}{\operatorname{\rk}}
\newcommand{\spann}{\operatorname{span}}
\newcommand{\Span}{\operatorname{Span}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\taut}{\operatorname{taut}} 
\newcommand{\Tor}{\operatorname{Tor}}
\newcommand{\Tr}{\operatorname{Tr}}
\newcommand{\tw}{\operatorname{tw}}
\newcommand{\Tw}{\operatorname{Tw}}
\newcommand{\wt}{\operatorname{wt}}
\newcommand{\SB}{\mathrm{SB}}
\newcommand{\CC}[1]{\left\llbracket #1 \right\rrbracket}
\newcommand{\bbar}{\boldsymbol{|}\hskip-2.5pt\boldsymbol{|}}

%%% suffix macros %%%

\newcommand{\dmod}{{\mathrm{-mod}}}   %% finitely-generated modules
\newcommand{\dgmod}{-\mathrm{dgmod}}
\newcommand{\fmod}{{\mathrm{-fmod}}}   %% finite-dimensional modules
\renewcommand{\pmod}{{\mathrm{-pmod}}}  %% fin-gen projective modules


%%% sub/superscript macros %%%

\newcommand{\opp}{\mathrm{op}}
\newcommand{\co}{\mathrm{co}}
\newcommand{\inv}{^{-1}}
\newcommand{\se}{^{(e)}}
\newcommand{\sh}{^{(h)}}
\newcommand{\dg}{\mathrm{dg}}	
\newcommand{\free}{\mathrm{free}}	
\newcommand{\tot}{\mathrm{tot}}
\newcommand{\gr}{\mathrm{gr}}


%%% very project specific macros %%%

\newcommand{\Ai}{A_\infty} 

\newcommand{\infone}{$(\infty,1)$}
\newcommand{\inftwo}{$(\infty,2)$}

\newcommand{\adeg}{\mathbf{a}}
\newcommand{\qdeg}{\mathbf{q}}
\newcommand{\tdeg}{\mathbf{t}}
\newcommand{\qbinom}[2]{\genfrac[]{0pt}{2}{#1}{#2}}

\newcommand{\vcomp}{\circ_2}
\newcommand{\Rouq}{F} % Rouquier complex
\newcommand{\ub}{\underline{\smash{\beta}}} % Braid word

\newcommand{\Ag}{\sigma} % Artin generator
\newcommand{\cohcat}{\mathrm{H}^*}
\newcommand{\htycat}{\mathrm{h}}
\newcommand{\Chb}{\operatorname{Ch^b}}
\newcommand{\Chbloc}{\operatorname{Ch^b_{loc}}}
\newcommand{\HChb}{\operatorname{\cohcat\Chb}}
\newcommand{\Kb}{\operatorname{K^b}}
\newcommand{\Kbloc}{\operatorname{K^b_{loc}}}
\newcommand{\truncK}{\operatorname{k^b}}
\newcommand{\Kbalt}{\mathrm{H}^0\Chb}

\newcommand{\cabledcross}{X}
\newcommand{\dgZ}{\mathcal{Z}^{\text{dg}}}
\newcommand{\AiZ}{\mathcal{Z}^{A_\infty}}
\newcommand{\barcx}{\mathbf{B}}

\newcommand{\Rtwo}{\mathrm{R2}}
\newcommand{\coRtwo}{\mathrm{coR2}}

\newcommand{\swap}{\mathrm{swap}}
\newcommand{\slide}{\mathrm{slide}}

\newcommand{\Vcat}{\mathcal{V}}
\newcommand{\Vcatt}{\Vcat^{\!\!\!\!\text{\tiny 2}}}
\newcommand{\Wcat}{\mathcal{W}}
\newcommand{\Wcatt}{\Wcat^{\!\!\!\!\text{\tiny 2}}}

\newcommand{\Vcattens}{\circledcirc}
\newcommand{\outtens}{\boxtimes}


\newcommand{\Vcatunit}{\oone_{\Vcat\Cat}}
\newcommand{\Vtwounit}{\oone_\Vtwocat}


\newcommand{\Cat}{\mathrm{Cat}}
\newcommand{\dgCat}{\mathrm{dgCat}}
\newcommand{\kCat}{\k\mathrm{Cat}}
\newcommand{\kCatt}{\k2\mathrm{Cat}}
\newcommand{\dgCatt}{\mathrm{dg}2\mathrm{Cat}}
\newcommand{\StrtwoCat}{\mathrm{Str2Cat}}
\newcommand{\Acat}{\mathcal{A}}
\newcommand{\Bcat}{\mathcal{B}}
\newcommand{\Ccat}{\mathcal{C}}
\newcommand{\Dcat}{\mathcal{D}}
\newcommand{\Ecat}{\mathcal{E}}
\newcommand{\Fcat}{\mathcal{F}}
\newcommand{\Tcat}{\mathcal{T}}
\newcommand{\Sets}{\mathrm{Sets}}

\newcommand{\Ccatun}{{\overline{\mathcal{C}}}}

%%% from GHW
\newcommand{\adds}{\Sigma}
\newcommand{\susp}[1]{\Sigma^{#1}}
\newcommand{\smMatrix}[1]{\left[\begin{smallmatrix}#1\end{smallmatrix}\right]}
\newcommand{\pretr}[1]{\operatorname{Pretr}(#1)}

%%% from LMGRSW
\newcommand{\oldD}{\mathrm{D}}
\newcommand{\oldDb}[1]{\oldD^b(#1)}
\def\bK{\mathbf K}
\newcommand{\K}{{\bK}}
\newcommand{\newKb}{\K^b}
\newcommand{\newKbloc}{\newKb_{\mathrm{loc}}}
\newcommand{\Hloc}{H_{\mathrm{loc}}}
\newcommand{\st}{\mathrm{st}}
\newcommand{\stkZ}{\st^{B\Z}_{\k}}
\newcommand{\stkBZ}{\stkZ}

%% structure for monoidal cats
\newcommand{\Vtens}{\otimes_{\Vcat}}
\newcommand{\Vunit}{\oone_\Vcat}
\newcommand{\Va}{\mathbf{a}}
\newcommand{\Vlunit}{\mathbf{l}}
\newcommand{\Vrunit}{\mathbf{r}}
\newcommand{\Vsym}{\mathbf{s}}
\newcommand{\RR}{\mathbf{R}}
%% structure for monoidal-cat-enriched-cats
\newcommand{\compmap}{m}
\newcommand{\idmap}{j}

%% structure for bicategories
\newcommand{\hcomp}{\circ_1}
\newcommand{\Bunit}{\oone_\Bcat}
\newcommand{\Ba}{\mathbf{a}}
\newcommand{\Blunit}{\mathbf{l}}
\newcommand{\Brunit}{\mathbf{r}}

%% structure for monoidal bicategories
\newcommand{\Vttens}{\otimes_{\Vcatt}}
\newcommand{\Bta}{a}
\newcommand{\Btlunit}{l}
\newcommand{\Btrunit}{r}
\newcommand{\Btptgn}{\pi}
\newcommand{\Btnu}{\nu}
\newcommand{\Btla}{\lambda}
\newcommand{\Btrh}{\rho}


%% structure for monoidal-bicat-enriched-bicats
\newcommand{\GSalpha}{\hat{\alpha}}
\newcommand{\GSsigma}{\hat{\sigma}}
\newcommand{\GStau}{\hat{\tau}}
\newcommand{\GSiota}{\hat{\iota}}
\newcommand{\GSmu}{\hat{\mu}}


\newcommand{\Ob}{\mathrm{Ob}}

\newcommand{\Vect}{\mathrm{Vect}}
\newcommand{\dgVect}{\mathrm{Vect}_\mathrm{dg}}
\newcommand{\gVect}{\mathrm{gVect}}
\newcommand{\dggVect}{\mathrm{gVect}_\mathrm{dg}}

% \newcommand{\st}{{\sf st}}
%\newcommand{\stkBZ}{\st^{B\Z}_{\k}}
%%%%%%%%%%% Environments %%%%%%%%%%%

\newtheorem*{maintheorem}{\hypertarget{thmA}{Main Theorem}}
\newtheorem*{thmA}{\hypertarget{oldthmA}{Theorem A}}
\newtheorem*{thmB}{\hypertarget{oldthmB}{Theorem B}}
%\renewcommand*{\themaintheorem}{\Alph{maintheorem}}
\newtheorem{byproduct}{Byproduct}[section]
\renewcommand*{\thebyproduct}{\alph{byproduct}}
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{theorem}[thm]{Theorem}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{conjecture}[thm]{Conjecture}
\newtheorem{hyp}[thm]{Hypothesis}
\newtheorem{hypothesis}[thm]{Hypothesis}
\theoremstyle{definition}
\newtheorem{defi}[thm]{Definition}
\newtheorem{definition}[thm]{Definition}
\newtheorem{construction}[thm]{Construction}
%\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{obs}[thm]{Observation}
\newtheorem{observation}[thm]{Observation}
\newtheorem{exas}[thm]{Examples}
\newtheorem{examples}[thm]{Examples}
\newtheorem{exa}[thm]{Example}
\newtheorem{example}[thm]{Example}
\newtheorem{nota}[thm]{Notation}
\newtheorem{conv}[thm]{Convention}
\newtheorem{warn}[thm]{Warning}
\newtheorem{notation}[thm]{Notation}
\newtheorem{convention}[thm]{Convention}
\newtheorem*{exa-nono}{Example}
\newtheorem*{thm-nono}{Theorem}
\newtheorem{thm-AB}{Theorem}

%%
\makeatletter
\newcommand{\mylabel}[2]{#2\def\@currentlabel{#2}\label{#1}}
\makeatother


%%%%%%%%%%% Maintenance %%%%%%%%%%%

\newcommand{\CaS}[1]{\textcolor[rgb]{0.60,0.00,0.50}{[CS: #1]}}%
\newcommand{\PW}[1]{\textcolor[rgb]{0.00,0.50,0.50}{[PW: #1]}}%
\newcommand{\todo}[1]{\textcolor[rgb]{0.00,0.00,0.80}{#1}}%
\newcommand{\outline}[1]{\textcolor[rgb]{0.80,0.00,0.00}{#1}}%
%\newcommand{\commented}[1]{}

%\usepackage{showkeys}%%%%%uncomment to enable showkeys
